Convergence and Running Time of Time-dependent Ant Colony Algorithms

Ant Colony Optimization (ACO) is a well-known method inspired by the foraging behavior of ants and is extensively used to solve combinatorial optimization problems. In this paper, we first consider a general framework based on the concept of a construction graph - a graph associated with an instance of the optimization problem under study, where feasible solutions are represented by walks. We analyze the running time of this ACO variant, known as the Graph-based Ant System with time-dependent evaporation rate (GBAS/tdev), and prove that the algorithm's solution converges to the optimal solution of the problem with probability 1 for a slightly stronger evaporation rate function than was previously known. We then consider two time-dependent adaptations of Attiratanasunthron and Fakcharoenphol's $n$-ANT algorithm: $n$-ANT with time-dependent evaporation rate ($n$-ANT/tdev) and $n$-ANT with time-dependent lower pheromone bound ($n$-ANT/tdlb). We analyze both variants on the single destination shortest path problem (SDSP). Our results show that $n$-ANT/tdev has a super-polynomial time lower bound on the SDSP. In contrast, we show that $n$-ANT/tdlb achieves a polynomial time upper bound on this problem.

==> content/Experiments.tex <==
%\section{Experimental Results}
%
%\todo[inline]{Jesse: update values in table when experiments are done running}
%\begin{table}
%\caption{Experimental comparison of $n$-ANT and $n$-ANT/tdlb. The convergence times written in bold
%text indicate the best combinations of algorithm with evaporation rate for the given value of $n$.
%Averages for a given $n$ are computed first over 50 independent runs on each sampled graph; subsequently
%this average convergence time is then again averaged over 100 independent sampled graphs.
%We cut off the simulation after
%$1000$ cycles; hence, we discard samples where any run of the algorithm reaches this limit.}
%\label{table: experiments}
%\begin{center}
%\begin{tabular}{ll*{10}{S[table-format=2]}} 
%\toprule 
%& & \multicolumn{10}{c}{Average convergence time for different $n$} \\ 
%\cmidrule{3-12} 
%\multirow{-2.5}{*}{\makecell{Algorithm}} & \multirow{-2.5}{*}{\makecell{$\rho$}} 
%& {10}& {20} & {30} & {40} & {50} & {60} & {70} & {80} & {90} & {100} \\ 
%\midrule
%$n$-ANT      & 0.1  & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\ 
%             & 0.01 & 22 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\ 
%             & 0.001 & 25 & 78 & 116 & 155 & 175 & 206 & 232 & 249 & & \\ \addlinespace
%$n$-ANT/tdlb & 0.1  & 22 & 53 & 76 & 100 & 122 & 147 & 157 & 176 & 188 & 210 \\ 
%             & 0.01 & 32 & 80 & 120 & 150 & 177 & 201 & 216 & $\times$ & 257 & \\ 
%             & 0.001 & 49 & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ & $\times$ \\ 
%\bottomrule 
%\end{tabular} 
%\end{center}
%\end{table}
%
%
%We compare the running time of $n$-ANT with $n$-ANT/tdlb on the single-destination shortest
%path problem (SDSP) in directed graphs. The graphs we consider are random graphs with
%random edge weights. To be precise: we sample graphs from $G(n, p_n)$, for
%$p_n = 2\log(n)/n$, and assign each edge of the sampled graphs a weight of 1. The value for $p_n$ is chosen so as to ensure that
%the sampled graphs are connected, but not so dense as to make the experiments too computationally expensive.
%
%On each sampled instance $G$, we run both $n$-ANT and $n$-ANT/tdlb. We set the target
%vertex arbitrarily before sampling the edges; by symmetry, the choice does not matter.
%We consider either algorithm to have converged if all ants have found their shortest
%paths to the target vertex (which we compute ahead of time using the Bellman-Ford algorithm).
%We then measure the number of cycles required by each algorithm to converge.
%Since these convergence times are random variables, we average them over multiple runs of the
%algorithm on different problem instances.
%
%One challenge in comparing the performance of these algorithms is in the different
%parameter choices. For $n$-ANT, we use $\tau_{\min{}} = 1/n^2$ and $\tau_{\max{}} = 1 - \tau_{\min{}}$;
%these are the values prescribed by Attiratanasunthron 
%and Fakcharoenphol~\cite{Attiratanasunthron2008running}. For $n$-ANT/tdlb, we use
%$\tau_{\max{}} = 1$.
%We then set $\tau_{\min{}}(m) = 1/\ln(m+1)$, in
%accordance with \Cref{sec:mmas specification}.
%
%It is less clear how to set the evaporation rate $\rho$. Attiratanasunthron 
%and Fakcharoenphol make no prescriptions for this parameter, except that it should be polynomially
%large to achieve a polynomial running time. We chose to evaluate both algorithms for several
%constant values of $\rho$, and determine the best combination of algorithm and evaporation rate
%for each $n$.
%The results of these experiments are displayed in \Cref{table: experiments}. 

%\subsection{Weighted Region Problem}
%
%The \emph{Weighted Region Problem} (WRP), introduced by Mitchell and Papadimitriou~\cite{mitchell1991weighted}, is one of the challenging optimization problems in various fields such as computer science, operations research, computational geometry, and geographic information systems.
%This problem involves finding the shortest path between two points on a plane divided into multiple polygonal regions, each assigned a non-negative number specifying the cost of travel through the region.
%An important theoretical result on WRP~\cite{de2014note} has shown that this problem cannot be solved in the algebraic computation model over the rational numbers (ACM$\mathbb{Q}$). In ACM$\mathbb{Q}$ it is possible to compute exactly any number that can be obtained from rational numbers by applying a finite sequence of operations from $+, -, \times, \div,$ and $\sqrt[k]{}$ (for any integral $k \geq 2$). This result justifies the search for approximate solutions as opposed to exact ones for WRP.
%
%{\color{red} This paragraph should be changed.}
%Motivated by the unsolvability result of WRP, we consider an \emph{ant colony optimization} (ACO) approach for this problem.
%This approach, introduced by Dorigo, Maniezzo and Colorini~\cite{dorigo1992optimization, dorigo1991ant}, which was inspired by analogies to the foraging behavior of real ant colonies, has been developed into a general and powerful metaheuristic with applications in various fields (see~\cite{dorigo2003ant}) since its introduction.
%To the best of our knowledge, WRP has never been approached by ACO. 
%
%
%\subsection{Other Problems?}
